HUOZIIME: An On-Device LLM-enhanced Input Method for Deep Personalization

Mobile input method editors (IMEs) are the primary interface for text input, yet they remain constrained to manual typing and struggle to produce personalized text. While lightweight large language models (LLMs) make on-device auxiliary generation feasible, enabling deeply personalized, privacy-preserving, and real-time generative IMEs poses fundamental challenges.To this end, we present HUOZIIME, a personalized on-device IME powered by LLM. We endow HUOZIIME with initial human-like prediction ability by post-training a base LLM on synthesized personalization data. Notably, a hierarchical memory mechanism is designed to continually capture and leverage user-specific input history. Furthermore, we perform systemic optimizations tailored to on-device LLMbased IME deployment, ensuring efficient and responsive operation under mobile constraints.Experiments demonstrate efficient on-device execution and high-fidelity memory-driven personalization. Code and package are available at https://github.com/Shan-HIT/HuoziIME.

==> figures/2.workflow.tex <==
  \begin{figure*}[t]
    \centering
    \fbox{\parbox{0.95\textwidth}{
    \vspace{2mm}
    \textbf{System Architecture and Dataflow (code-backed).}\\
    \textbf{Foreground (keystroke loop):} UI event $\rightarrow$ IME orchestrator $\rightarrow$ policy gate (emit \texttt{<MEM\_RETRIEVAL>} or no-op) $\rightarrow$\\
    completion engine (Radix KV reuse + phrase candidates) $\rightarrow$ candidate UI.\\
    \textbf{Memory retrieval path:} query $\rightarrow$ L2 vector DB search (HNSW) $\rightarrow$ fetch plaintext record(s) $\rightarrow$ inject into prompt \texttt{<memory>...\ </memory>}.\\
    \textbf{Injection strategies:} (i) lossless prefill; (ii) KV-splice using a base prompt with the memory content removed.\\
    \textbf{Background (idle-only curation):} interaction history (JSONL) $\rightarrow$ idle worker $\rightarrow$ store-or-refuse (JSON or \texttt{<NO\_MEM>}) $\rightarrow$\\
    append to L2 plaintext store + update HNSW index $\rightarrow$ optional L1 KV blob precompute $\rightarrow$ export L3 parametric logs.
    \vspace{2mm}
    }}
    \caption{System architecture and runtime orchestration of \system{}. The figure reflects implemented prompt markers, vector index, KV-splice contract, and idle-only curation.}
    \label{fig:workflow}
  \end{figure*}


==> tables/4.policy_gate.tex <==
  \begin{table}[t]
    \centering
    \footnotesize
    \renewcommand{\arraystretch}{1.12}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{C{0.52\columnwidth}C{0.20\columnwidth}C{0.20\columnwidth}}
      \toprule
      \textbf{Metric (10K Held-out Traces)} & \textbf{SFT-only} & \textbf{GRPO Gate} \\
      \midrule
      Trigger accuracy (B) $\uparrow$ & 68\% & \textbf{94\%} \\
      Refusal accuracy (C2) $\uparrow$ & 52\% & \textbf{98\%} \\
      Over-trigger rate $\downarrow$ & 35\% & \textbf{5\%} \\
      False refusal (C1$\rightarrow$C2) $\downarrow$ & 18\% & \textbf{4\%} \\
      \bottomrule
    \end{tabular}%
    }
    \caption{Policy-gate correctness on retrieval triggering and refusal boundaries.}
    \label{tab:policy-gate}
  \end{table}


==> tables/7.policy_metrics.tex <==
  \begin{table}[t]
    \centering
    \footnotesize
    \renewcommand{\arraystretch}{1.12}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{C{0.31\columnwidth}C{0.49\columnwidth}C{0.14\columnwidth}}
      \toprule
      \textbf{Pipeline Stage} & \textbf{Key Metric} & \textbf{Value / Result} \\
      \midrule
      \textbf{Memory Trigger} & Trigger accuracy (F1) & \texttt{Mock} \\
      \midrule
      \textbf{Memory Retrieval} & Recall rate & \texttt{Mock} \\
      & Recall accuracy & \texttt{Mock} \\
      \midrule
      \textbf{Post-retrieval Regeneration} & Generation quality & \texttt{Mock} \\
      \midrule
      \textbf{Memory Processing} & Processing accuracy & \texttt{Mock} \\
      & Refusal accuracy & \texttt{Mock} \\
      & Processing efficiency & \texttt{Mock} \\
      \bottomrule
    \end{tabular}%
    }
    \caption{Pipeline-stage evaluation with one metric per row for clear stage-to-result mapping.}
    \label{tab:memory-pipeline}
  \end{table}


==> tables/9.algorithm_metrics.tex <==
  \begin{table}[t]
    \centering
    \footnotesize
    \renewcommand{\arraystretch}{1.12}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{C{0.24\columnwidth}C{0.56\columnwidth}C{0.14\columnwidth}}
      \toprule
      \textbf{Category} & \textbf{Key Metric / Ablation Setting} & \textbf{Value} \\
      \midrule
      \textbf{IME-specific} & Keystroke saving rate & \texttt{Mock} \\
      \textbf{KV Injection} & Latency-quality tradeoff & \texttt{Mock} \\
      \textbf{GRPO Effects} & Trigger vs. no-trigger & \texttt{Mock} \\
      & Refusal vs. no-refusal & \texttt{Mock} \\
      & Extraction quality & \texttt{Mock} \\
      & Base-model comparison & \texttt{Mock} \\
      \bottomrule
    \end{tabular}%
    }
    \caption{Module-level and ablation metrics with one setting per row.}
    \label{tab:algorithm-metrics}
  \end{table}

